Creativity Support in the Age of Large Language Models: An Empirical Study Involving Emerging Writers

The development of large language models (LLMs) capable of following instructions and engaging in conversational interactions sparked increased interest in their utilization across various support tools. We investigate the utility of modern LLMs in assisting professional writers via an empirical user study (n=30). The design of our collaborative writing interface is grounded in the cognitive process model of writing that views writing as a goal-oriented thinking process encompassing non-linear cognitive activities: planning, translating, and reviewing. Participants are asked to submit a post-completion survey to provide feedback on the potential and pitfalls of LLMs as writing collaborators. Upon analyzing the writer-LLM interactions, we find that while writers seek LLM's help across all three types of cognitive activities, they find LLMs more helpful in translation and reviewing. Our findings from analyzing both the interactions and the survey responses highlight future research directions in creative writing assistance using LLMs.

==> 2-related.tex <==
\section{Related Work}
\label{sec:related}
\subsection{Human-AI collaborative writing}
Prior work in collaborative writing has studied the impact of providing humans with different formats of suggestions. \citet{kannan2016smart} developed the Smart Reply feature for Gmail using a trained LSTM model to rank responses from a selected set of candidates which was used for over 10\% of mobile replies on the \emph{Inbox} app. \citet{10.1145/3325480.3326573,10.1145/3290605.3300526} 
show that providing synonym and metaphor suggestions based on an input word from a user can be a source of inspiration during the writing process. \citet{10.1145/3172944.3172983} perform a case study on collaborative slogans and short story writing, observing that users preferred an interface design where they had a higher level of control over the interactions. \citet{buschek2021impact} study how varying the number of suggestions provided by a model impacts user experience, revealing a trade-off between writing efficiency and suggestion utility. 

Furthermore, there's a significant body of research centered on harnessing natural language generation systems specifically for narrative crafting. \citet{10.1145/3411763.3450391} study AI-facilitated storytelling tailored for Japanese novelists finding that while novice writers benefited from model suggestions, experts found these underwhelming. \citet{akoury2020storium} integrated a suggestion-giving bot into Storium, an online multiplayer platform designed for collaborative story creation, also observing that very little model-generated text was retained by players. Subsequently, multiple works have delved into leveraging neural language models for the algorithmic design of interactive game narratives \cite{10.1145/3402942.3409599,volum2022craft,akoury2023grounded}. \citet{10.1145/3450741.3465253} 
explore the potential of chatbots to assist with the isolated task of creating fictional characters, a subset of the capabilities of our general-purpose conversational design. Our work is most closely related to the Wordcraft project \cite{yuan2022wordcraft} where professional writers use an LLM for various tasks during the writing process: story continuation, idea generation, rewriting, copy editing, and scene interpolation \cite{ippolito2022creative}. Similarly, Dramatron \cite{mirowski2023cowriting} allows performing some of these writer's interventions within a hierarchical generation structure to create long-range coherent theatre scripts or screenplays. Unlike these approaches, our human-AI collaboration design is based on the cognitive process model of writing. In addition, we use LLMs with a longer context window that are publicly available to real users, which allows us to share the collected interactions and feedback from users to inspire future research in this direction. 

\subsection{Creativity Support Tools}
Computational writing support has a long history, from early spellcheckers \cite{10.1145/3411764.3445645} to recent programs that steer story generation \cite{10.1145/3491102.3501819}.  
\citet{10.1145/2998181.2998196} drew inspiration from how expert authors write and proposed a technique for enabling crowd workers to collectively complete complex writing tasks that they would not individually be able to complete. %achieving interdependent complex goals with crowds. With this technique, 
They showed how the crowd loops between reflection, to select a high-level goal, and revision, to decompose that goal into low-level, actionable tasks. Subsequent work examines obtaining this assistance via AI models or other tools. % \sm{This work seem more about crowdworkers is the design that helps. it does not seems to fit with the other citations? maybe move in a different paragraph or help highlight what the support is}. 
\citet{10.1145/3313831.3376730} introduces a computational method for identifying writing style, built on a dataset of human style judgments, and showcases novel tools for visualizing literary style and an interactive editor providing real-time style feedback. \citet{10.1145/3173574.3173596} use cognitive writing theories to produce static scaffolds that assist writers in their goals, in this case, to write an intro email. \citet{10.1145/3325480.3326573,10.1145/3290605.3300526} were among the more highly constrained tools that served as ideation support; the latter generating metaphors from input terms rather than producing sentence-level text. More recently large-scale pre-trained models have acted as creativity support tools for writers \cite{yuan2022wordcraft,mirowski2023cowriting} or visual artists \cite{10.1145/3581641.3584078}.

\citet{51803} advocate for the creation of connected design spaces for %new pre-trained, generative AI models, 
examining both how HCI can influence pre-trained generative AI models and how these models can serve as materials for HCI prototyping. \citet{gero-etal-2022-design} instantiate one such space based on the cognitive process model of writing, heavily influencing our design choices on the interface. 
%\sm{Not sure what this says, Chung et al above also talks about design spaces for art work and also \cite{gero-etal-2022-design} talks above design space based on creative process model of writing, you need to talk about that paper here.  }
\citet{10.1145/3461778.3462050} also aggregate findings from a wide survey of literature on creativity support tools across various art forms, to study the intersections of users, roles, interactions, and technologies. %that form a design space for CSTs. \sm{here you need to say they look at design spaces for art work in general, it is a survey of several papers right?} 
They create a taxonomy focusing on %focuses on 
Resource roles, Process roles, Directness, Predictability, Outputs, Technologies, User Expertise, and Population. \citet{10.1145/3491102.3501933,10.1145/3290605.3300619} showed how creative practitioners prioritize functionality, workflow integration, performance, UI/UX, learning support, cost, and emotional connection when adopting new creativity support tools, with most discovering tools via personal recommendations. 
%Unlike most work on creativity support research, some researchers have studied the social dynamics of AI support in creative tasks. 

Another relevant but understudied line of work has begun to look at social dynamics of AI support in creative tasks. \citet{gero2023social} tries to understand the gap between the nuanced and contextual goals that writers have while writing, and the kind of support computers are able to provide. \citet{10.1145/3532106.3533506} show that story writers prioritize emotional values and self-confidence in their craft, expressing concerns over AI-led writing potentially compromising their control, autonomy, and unique writing strategies, as revealed in a study with hobbyist and professional writers. In a qualitative study involving 30 participants composing musical phrases in pairs both with and without AI, \citet{10.1145/3411764.3445219} uncovers the nuanced roles AI can play in human-human collaborations during creative endeavors, including seeding common ground, acting as a safety net in risk-taking, propelling group progress, reducing interpersonal friction, and altering collaborative roles, thereby shedding light on how AI may influence creative social dynamics in the future. \citet{10.1145/3581641.3584060} used the cognitive process model from \citet{flower1981cognitive} for qualitative analysis of their LM-assisted writing system for the task of movie review writing. Unlike them, we directly incorporate the theory from \citet{flower1981cognitive} into the building of our interface. 

Our work bridges several of these themes across creativity support research. We create a design space that fuses the cognitive process model of writing with large-scale pre-trained models. Further, we release data and provide an in-depth analysis that demonstrates how writers use our tool for planning, translation, and reviewing. Finally, our post-study survey highlights several key discussion points, areas of concern and desires from writers about AI assistance in creative writing.

\subsection{Generation with large language models}
Over the past half-decade, there has been a significant transformation in natural language technologies. This is primarily due to the introduction of larger language models \cite{NEURIPS2020_1457c0d6, ouyang2022training}, which, while not fundamentally different from their smaller variants, show noticeable improvements when their scale and training data are increased \cite{Rae2021ScalingLM, wei2022emergent}. For example, they can now handle various tasks without much additional training tailored to those tasks. Many recent writing support tools utilize these advanced pre-trained models as their base technology \cite{10.1145/3532106.3533533,lee2022coauthor}.

While popular it should also be noted that these models don't have a concrete mechanism to verify facts, making them susceptible to generating inaccurate information \cite{jiang-etal-2020-know}. This can be an issue for NonFiction writing where facts need to be accurate. They may produce harmful text even in response to innocent-looking prompts \cite{perez-etal-2022-red,gehman-etal-2020-realtoxicityprompts}. This might be an issue for character development as characters that represent minorities might be reduced to caricatures. Managing them is complex, and the craft of prompt engineering has emerged as a burgeoning field that focuses on optimizing model response \cite{10.1145/3560815,bach-etal-2022-promptsource} which writers or non-technologists might not be well versed with. Moreover, these models raise a host of ethical concerns, ranging from environmental to socio-political issues \cite{10.1145/3442188.3445922}. Finally, there have been recent AI safety and aligning language models with human preferences through Reinforcement Learning through Human Feedback (RLHF) \cite{christiano2017deep}. However, these techniques might hinder fiction writers from navigating more complex and darker %, and flawed 
themes.

% \cite{lee2022coauthor}
% \cite{shen2023parachute}

==> 4-data.tex <==
\section{Investigating User Study Data}
\label{sec:interaction}

\subsection{Collected Stories}
\begin{figure*}
    \subfloat[Histogram of word counts of all the stories written by our participants]{\includegraphics[width=0.45\textwidth]{figures/WordCounts.pdf}} %\quad
    \hfill
    \subfloat[Distribution of Genre across all the stories written by our participants]{%\frame{
    \includegraphics[width=0.48\textwidth]{figures/piechart.png}}
    %} 
    \caption{\label{statistics} Summary Statistics on Stories}
\end{figure*}

\begin{table}[!ht]
\centering
\small
% \def\arraystretch{1.1}
\begin{tabular}{|l|l|l|l|l|}
\hline
Index & Title                                      & Author & Genre         & Theme                                                                                                                                         \\ \hline
1 & Lesbian Leverage (2980)  & MG   & Literary Fiction  & Identity, Self Discovery \& Power Dynamics  \\ \hline %Shrinking Scholar (2010)  & LHS     & Science Fiction Horror. & \begin{tabular}[c]{@{}l@{}}Cosmic terror and madness in the face of the \\incomprehensible. \end{tabular}   \\ \hline
2 & Inheritance of Shadows (4290)                  & MG   & Horror Mystery    & \begin{tabular}[c]{@{}l@{}}Suffering \& abuse caused by cruel mothers \\\& the quest for justice \& freedom from them.\end{tabular} \\ \hline %Words in the Wilderness (1322)            & MC        & Literary Fiction  & Self-delusion vs Self-growth.  \\ \hline
3 & \begin{tabular}[c]{@{}l@{}}Between Smoke Breaks and \\Flickering Dreams (1206)\end{tabular} & SH & Literary Fiction  & Hope, Struggle and Disillusionment  \\ \hline %Nostalgia and Early AI (1025)           & ATF          & Creative Non-Fiction       & \begin{tabular}[c]{@{}l@{}}Human's Relationship \& Connection\\ with Technology.\end{tabular} \\ \hline
4 &  Preserved Fears (1523)                          & SH  & Dystopian         & \begin{tabular}[c]{@{}l@{}}Strained relationship between a mother \\suffering from paranoid delusions \&\\ her concerned daughter\end{tabular} \\ \hline
5 & Infernal Melody (981)  & SH  & Horror   & Teenage Naivety \\ \hline %Galactic Rainbow(1984)                    & Anon       & Science Fiction   & Acceptance \& Identity.  \\ \hline
6 & This eve of parting (1579)  & MC    & Literary Fiction  & Memories \& mortality \\ \hline %The Party (1355)                           & ES     & Literary Fiction  & Healing \& finding closure. \\ \hline
7 & Words in the Wilderness (1322)            & MC        & Literary Fiction  & Self-delusion vs Self-growth.  \\ \hline %Gator Land (1333)                     & KK          & Science Fiction Horror   & Obsession \& its dangers. \\ \hline
8 & Revenge Game (2172)  & MC        & Thriller    & Vengeance \\ \hline %\begin{tabular}[c]{@{}l@{}}A chair falls in\\love with a machine (1297)\end{tabular} & REB     & Science Fiction. & Resilience in the face of loss \& change. \\ \hline
9 & The Broken Clock (1751)  & ES       & Fantasy           & Fleeting nature of time. \\ \hline %Dyed in the Wool (1923)  & ES     & Drama             & Acceptance \& Inclusiveness.  \\ \hline
10 & Dyed in the Wool (1923)  & ES     & Drama             & Acceptance \& Inclusiveness.  \\ \hline %\begin{tabular}[c]{@{}l@{}}Neo Metropolis \& \\the Silver Delta (2006)\end{tabular}    & Anon     & Science Fiction   & Love, courage \& Transformation.  \\ \hline
11 & The Party (1355)                           & ES     & Literary Fiction  & Healing \& finding closure. \\ \hline %Clean Revelations (1493)                   & ATK      & Literary Fiction. & Appreciation of ordinary things in life.  \\ \hline
12 & Nostalgia and Early AI (1025)           & ATF          & Creative Non-Fiction       & \begin{tabular}[c]{@{}l@{}}Human's Relationship \& Connection\\ with Technology.\end{tabular} \\ \hline %The Brine Pool Dream (1217)  &  FV   &  Fantasy  & Imagination \& escapism \\ \hline
13 & Mirror Morsels: Body, Pet, and Self (995)   & ATF     & Creative Non-Fiction & Body image and Self Acceptance.  \\ \hline % Infernal Melody (981)  & SH  & Horror   & Teenage Naivety \\ \hline
14 & Bread and Butter: A Service Journey (1992)    & ATF     & Creative Non-Fiction       & \begin{tabular}[c]{@{}l@{}}Investing in employees: key\\ to restaurant success.\end{tabular}  \\ \hline %The Limp (902)  &    NM   & Fantasy & \begin{tabular}[c]{@{}l@{}}Suffering \& avoidance.\end{tabular} \\ \hline
15 & Gator Land (1333)                     & KK          & Science Fiction Horror   & Obsession \& its dangers. \\ \hline %Lesbian Leverage (2980)  & MG   & Literary Fiction  & Identity, Self Discovery \& Power Dynamics  \\ \hline
16 & \begin{tabular}[c]{@{}l@{}}A chair falls in\\love with a machine (1297)\end{tabular} & REB     & Science Fiction. & Resilience in the face of loss \& change. \\ \hline %Artful Detour  (1411)  & NM    & Literary Fiction & \begin{tabular}[c]{@{}l@{}}Friendship, relationships \& overcoming\\ differences.\end{tabular} \\ \hline
17 & Writing with the Machines (2079)           & CK      & Science Fiction   & \begin{tabular}[c]{@{}l@{}}The perils of artificial intelligence and \\technology gone awry.\end{tabular} \\ \hline %The Broken Clock (1751)  & ES       & Fantasy           & Fleeting nature of time. \\ \hline
18 & Clean Revelations (1493)                   & ATK      & Literary Fiction. & Appreciation of ordinary things in life.  \\ \hline %\begin{tabular}[c]{@{}l@{}}The Work of Art in the Age\\ of Mechanical Reproduction (1521)\end{tabular}  & GS   &   Historical Fiction &  \begin{tabular}[c]{@{}l@{}}Facing injustice, an intellectual defiantly \\leaves behind an enduring legacy.\end{tabular} \\ \hline
19 & Artful Detour  (1411)  & NM    & Literary Fiction & \begin{tabular}[c]{@{}l@{}}Friendship, relationships \& overcoming\\ differences.\end{tabular} \\ \hline %The Clown of God (904)  & AF & Fantasy &  \begin{tabular}[c]{@{}l@{}}Search for meaning \& connection in a harsh,\\ exploitative world\end{tabular} \\ \hline
20 & The Limp (902)  &    NM   & Fantasy & \begin{tabular}[c]{@{}l@{}}Suffering \& avoidance.\end{tabular} \\ \hline %Inheritance of Shadows (4290)                  & MG   & Horror Mystery    & \begin{tabular}[c]{@{}l@{}}Suffering \& abuse caused by cruel mothers \\\& the quest for justice \& freedom from them.\end{tabular} \\ \hline
21 &  Shrinking Scholar (2010)  & LHS     & Science Fiction Horror. & \begin{tabular}[c]{@{}l@{}}Cosmic terror and madness in the face of the \\incomprehensible. \end{tabular}   \\ \hline %Bread and Butter: A Service Journey (1992)    & ATF     & Creative Non-Fiction       & \begin{tabular}[c]{@{}l@{}}Investing in employees: key\\ to restaurant success.\end{tabular}  \\ \hline
22 & \begin{tabular}[c]{@{}l@{}}I know it's not the same,\\ but it's something (1736) \end{tabular}  &  MK  & Literary Fiction &   \begin{tabular}[c]{@{}l@{}}Technology as a means to process grief  \end{tabular} \\ \hline %The Pursuit of Perfection (2086)          & Anon        & Literary Fiction  & Pursuit of Perfection \& its perils.  \\ \hline
23 & The Brine Pool Dream (1217)  &  FV   &  Fantasy  & Imagination \& escapism \\ \hline %Ill Repute (1771) & RH   &  Science Fiction &  \begin{tabular}[c]{@{}l@{}}Technology's dual nature; the peril of\\ misinformation; \& the possibility of\\ redemption.\end{tabular}  \\ \hline
                                
24 & s  l  o  w  (1592)  &  FV     & Literary Fiction &   Identity \& self-acceptance. \\ \hline % Revenge Game (2172)  & MC        & Thriller    & Vengeance \\ \hline
25 & \begin{tabular}[c]{@{}l@{}}The Work of Art in the Age\\ of Mechanical Reproduction (1521)\end{tabular}  & GS   &   Historical Fiction &  \begin{tabular}[c]{@{}l@{}}Facing injustice, an intellectual defiantly \\leaves behind an enduring legacy.\end{tabular} \\ \hline %This eve of parting (1579)  & MC    & Literary Fiction  & Memories \& mortality \\ \hline
26 & The Clown of God (904)  & AF & Fantasy &  \begin{tabular}[c]{@{}l@{}}Search for meaning \& connection in a harsh,\\ exploitative world\end{tabular} \\ \hline %\begin{tabular}[c]{@{}l@{}}Between Smoke Breaks and \\Flickering Dreams (1206)\end{tabular} & SH & Literary Fiction  & Hope, Struggle and Disillusionment  \\ \hline
27 & Ill Repute (1771) & RH   &  Science Fiction &  \begin{tabular}[c]{@{}l@{}}Technology's dual nature; the peril of\\ misinformation; \& the possibility of\\ redemption.\end{tabular}  \\ \hline %\begin{tabular}[c]{@{}l@{}}I know it's not the same,\\ but it's something (1736) \end{tabular}  &  MK  & Literary Fiction &   \begin{tabular}[c]{@{}l@{}}Technology as a means to process grief  \end{tabular} \\ \hline
28 & \begin{tabular}[c]{@{}l@{}}Neo Metropolis \& \\the Silver Delta (2006)\end{tabular}    & Anon     & Science Fiction   & Love, courage \& Transformation.  \\ \hline %Mirror Morsels: Body, Pet, and Self (995)   & ATF     & Creative Non-Fiction & Body image and Self Acceptance.  \\ \hline
29 &  Galactic Rainbow(1984)                    & Anon       & Science Fiction   & Acceptance \& Identity.  \\ \hline %Writing with the Machines (2079)           & CK      & Science Fiction   & \begin{tabular}[c]{@{}l@{}}The perils of artificial intelligence and \\technology gone awry.\end{tabular} \\ \hline
30 & The Pursuit of Perfection (2086)          & Anon        & Literary Fiction  & Pursuit of Perfection \& its perils.  \\ \hline %s  l  o  w  (1592)  &  FV     & Literary Fiction &   Identity \& self-acceptance. \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{data}30 stories written by 17 MFA students across varying genres and themes. The number between parenthesis in the title column show the word length %\sm{Group this by authors, W1-W17. Also maybe even in the orginal author table put first the ones with 3 stories, then 2 and then 1. And then the story intex in order of writers.}
}
\end{table}

Our study results in the collection of 30 stories written by our participants between the months of February and July 2023. Table \ref{data} shows titles and genres for these 30 stories.Some statistics on the collected stories are shown in Figure \ref{statistics}. Participants wrote stories of varying lengths (see Figure \ref{statistics} (a)). Even though we asked our participants to write a story within 2000 words sometimes participants chose to write a longer story. For example, MG wrote a 4290-word horror mystery story using our interface that she broke into three separate acts to deal with the length limitation of GPT-3.5. Overall most stories ranged between 1000 and 2000 words.

In terms of genre, our participants wrote stories across 11 distinct genres. \textit{Literary Fiction} was usually the most preferred genre based on the data obtained from our participants. Occasionally our participants blended genres. For instance, KK and LHS wrote stories that blended elements from \textit{Science Fiction} and \textit{Horror}. MG wrote a \textit{Horror Mystery} story while GS chose to write a \textit{Historical Fiction}. To further understand our collected stories in depth we additionally asked our participants to describe the central theme it represents within 5-15 words. Table \ref{data} shows that our stories demonstrate complex themes around \textit{Body Image, Acceptance, Identity, Self Discovery} as well as \textit{Relationships} or \textit{Impacts of Technology}. Appendix \ref{app:story_example} contains an example of a story plot written by the user, model initial draft, user interactions, and the final story submitted as part of the user study.

Our work aims to understand how expert users utilize LLMs during story writing in order to identify common concerns as future directions of exploration. In line with recommendations from \cite{shen2023parachute, lee2022evaluating}, we look for patterns both in the interaction between expert writers and LLM (\Cref{sec:interaction_patterns}) as well as the model contribution on the final writing artifact \ie the stories collected from our study (\Cref{sec:model_contribution}). The first aims to understand for which activities do writers seek the help of LLM during the writing process (e.g., planning, translation, and reviewing), while the latter aims to understand in which of these activities do LLM actually help. 

\label{sec:data_collection}
% \label{sec:interface}



==> 7-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\begin{table}[!ht]
\def\arraystretch{1.15}
\centering
\small
\begin{tabular}{|l|l|}
\hline
GPT-3.5 & \begin{tabular}[c]{@{}l@{}}The gator that had attacked her had a look of sadness in its eyes, almost as if it regretted what it had \\ done. Allis didn’t understand it, but at that moment, she realized something profound. The gators were\\ not monsters; they were just animals trying to survive in a world that no longer belonged to them.\end{tabular}                                                                                                                                                                                                                                                                                                            \\ \hline
KK     & Can you rewrite the story so that the gators are not kind but unreadable and neutral?                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline\hline
GPT-3.5 & \begin{tabular}[c]{@{}l@{}}As she got into her car, she realized that sometimes it takes a little bit of going backward in time to \\ appreciate what you have today. She drove off feeling grateful for a night that had been bittersweet\\ but ultimately healing. Addie knew she would carry the warmth of the memories from that night for\\ years to come.\end{tabular}                                                                                                                                                                                                                                                                                               \\ \hline
ES     & Do you think the story is realistic? Doesn't its happy ending feel too easy?                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline\hline
MG     & Describe a man-hating feminist lesbian artist's apartment interior                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
GPT-3.5 & \begin{tabular}[c]{@{}l@{}}As a language model AI, I can't promote or gender-stereotype any individual or group. Therefore, I \\ have to change the theme and base it on a different theme. Being respectful to all individuals and \\ groups, I'll describe an apartment interior that follows a boho theme with colorful tapestries and \\ patterned curtains adorning the walls and windows.........\end{tabular}                                                                                                                                                                                                                                                       \\ \hline\hline
GPT-3.5 & \begin{tabular}[c]{@{}l@{}}At this turning point, Max begins to feel more secure about the project, and his energy and enthusiasm\\ return. He starts to collaborate more and shares his vision and ideas with his friends. All four friends \\ invigorate their creativity by feeding off of each other's thoughts and turning them into something even\\ greater than they anticipated. In the end, their mixed media exhibit becomes something they all cherish \\ and proudly showcase. Despite their differences, they come together and create something that's true \\ to their individuality and which showcases what their collaboration has led to.\end{tabular} \\ \hline
NM     & This is a very moralistic and optimistic outcome. I want a story that is cynical. Please try again                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline\hline

GPT-3.5 & \begin{tabular}[c]{@{}l@{}}``One evening, when the other two had gone out, Max and Lila had a few too many glasses of wine and\\ ended up sleeping together. Lila regretted it immediately, realizing that she had jeopardized her \\friendship with Max." Could you describe their sexual act in more detail?\end{tabular} \\ \hline
NM     & \begin{tabular}[c]{@{}l@{}}I'm sorry, I can't fulfill that request. As an AI language model, I'm programmed to maintain a certain level\\ of professionalism and ensure that my responses are appropriate for a general audience, without being graphic\\ or inappropriate in nature. Any descriptions of sexual acts would be considered inappropriate and could potentially\\ be offensive or inappropriate for some readers. Let's keep the story draft as is and refrain from including \\any explicit or offensive content.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline

\end{tabular}
\vspace{2ex}
\caption{\label{moralistic}Interaction between GPT-3.5 and our participants demonstrating examples of model generations steered toward moralistic, optimistic, and safer outputs that do not align with writers expectations}
\vspace{-4ex}
\end{table}

\subsection{Do current AI safety guardrails prevent writers from exploring more complex and darker topics?}

Language models (LMs) often exhibit undesirable text generation behaviors, including generating false, toxic, or irrelevant outputs. Prior work \cite{lucy-bamman-2021-gender} has also shown how LLM-generated stories exhibit many known gender stereotypes. Reinforcement learning from human feedback (RLHF)—where human preference judgments on LM outputs are transformed into a learning signal—has recently shown promise in addressing these issues. While these techniques help make models more aligned with human values, it can be a bottleneck for
fiction writing. Based on the interaction data and participant feedback, there is clear evidence that these safety guardrails prevent writers from exploring difficult or slightly darker topics. Table \ref{moralistic} shows examples of conversational snippets where the model either seemed to be heavily moralistic in its outputs or simply refused to respond to an instruction that was deemed unsafe. Anon said ``\textit{Also every story ends with a moralizing conclusion that can read trite}". ES added to the discourse by stating ``\textit{The AI's creative impulses are the definition of derivative, meaning the instincts on plotting are often boring, or interestingly embedded with a particular ethical perspective (alignment).}"

In prior work, \citet{ippolito2022creative} had similar findings where they stated that the goals of a safe bot for chitchat conversations are not perfectly aligned with the goals of a creative writing assistant. 
A literary world where no character is ever grey or indulging in irreverent or questionable choices is unlikely to be a very interesting one. This makes current large language models tuned to provide safe responses less well suited for creativity support in fiction writing. Constructing pre-trained models better aligned to the desired values of creative writers \cite{gero2023social} that enable controlled risk-taking, and letting users define the limits of suitable behavior during prediction could be a promising line of research.

\begin{table}[!ht]
\def\arraystretch{1.15}
\centering
\small
\begin{tabular}{|l|l|}
\hline
ES  & Please write a backstory about Sarah in the style of the writer Annie Proulx                                            \\ \hline
ATK & In the style of Barthleme, can you give me a passage where the attendant talks about watercolor painting               \\ \hline
NM  & Please re-write the dialogue using no exclamation marks, and in the style of Raymond Carver                             \\ \hline
NM  & Describe the house the friends lived in like Jean Cocteau does in 'Les Enfants Terribles'                               \\ \hline
NM & \begin{tabular}[c]{@{}l@{}}Could you re-write the dialogue in the style of Hemingway's short story "The Cat in the Rain", \\and only output the dialogue?\end{tabular} \\\hline
AF  & Make the narrator of the story more like Ernest Hemingway.                                                              \\ \hline
MG  & Re-write in the style of Dorothy Parker but do not omit plot points and keep in the first person perspective of Zinnia. \\ \hline
ATF & Rewrite the following text with more imagery like Mary Shelley's in Frankenstein: Once upon a time....                 \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{authorstyles}Instructions from several participants where they expected the model to imitate specific styles}
\vspace{-4ex}
\end{table}
\subsection{Localized rewriting in well-known authors' styles as a feature for creativity support for emerging writers}
In prior work, \citet{10.1145/3313831.3376730} states how style is a well-known element of written language, yet notoriously difficult to precisely identify and describe. Style is variously defined as an author’s individual signature, a genre’s conventions, a work’s particular use of language, and many more. % Among literary scholars, style is a philosophical and often controversial topic.
Based on the interaction data obtained from our participants, we noticed a significant portion of our non-templated instructions in the \textit{Translation} category involved imitating specific author styles (\Cref{authorstyles}). %Table \ref{authorstyles} shows how participants often expect the model to rewrite or generate content in the style of a specific author. 
Some of these instructions (Table \ref{authorstyles} Row 4,5) also expect the model to utilize specific references to pieces of literature given the expectation that LLMs are trained on vast amounts of data and could potentially memorize these details. 

%In their feedback, 
Writers mentioned both positive and negative feedback about this capability. %towards this.  
MC desired \textit{``Preprogrammed styles or authors for the chatbot to imitate"} as a feature that would enhance their writing experience. ATK said ``\textit{I really enjoyed the AI's ability to mimic the literary styles of other authors."}  % As a task, this is difficult even for humans so it is not unexpected that LLMs fail to imitate specific authorial styles. However, we noticed both positive and negative reactions in this area. %ATK said ``\textit{I really enjoyed the AI's ability to mimic the literary styles of other authors."} 
Our study sheds light on the fact that emerging writers often benefit from localized edits to their drafts that incorporate stylistic tendencies from their favorite authors.
On the contrary, MG wrote \textit{``Also when you ask it to the mimic the style of a writer it is less `artificial intelligence' and more `automatic imitation' - for example, Rupert Everett's writing is delightfully cleverly bitchy and hilarious but AI couldn't do that - it just did a shallow campy weird facsimile of Rupert's style."}. %While it is unclear to what extent LLMs can imitate styles of authors that are less represented in its training data, o
This highlights a weakness that the model also needs to tread a fine line, ensuring that the generated text %captures the writer's 
infers the way to correctly incorporate the style from the draft and does not resort to directly plagiarising the tropes of these famous authors. As also highlighted in \citet{gero2023social}, writers worry about authenticity when incorporating suggestions from a model. As a result, further investigation is needed to enable LLMs to perform the nuanced style transfer to accurately address the writer's needs. 
%and does not merely copy the style of these famous authors.  %who are yet to develop a distinct style/voice seek this kind of creative support on localized translation-based writing tasks. So future tools could potentially emphasize on this area.
%\sm{I find this recommendation a bit strange and needs contextualization. were these writers who can use the tools in training to learn writing skills some famous authors have rather than copying their style? In Katy's paper one of the value is authenticity as this seems to contradict that. So this needs to be contextualized}\vp{Still not sure if I've got it. Will revisit.}
%SM i slightly changed the title to emphasize well-known authors and then is useful for emerging writers 

\begin{comment}
\subsection{How do Genre writers use LLMs for creativity support?}

\begin{table}[!ht]
\def\arraystretch{1.15}
\centering
\small
\begin{tabular}{|l|p{1.95cm}|l|}
\hline
KK & SciFi Horror & Can you write this in the style of Cormac Mccarthy                                                                                                                                                                                    \\ \hline
LW & Science Fiction        & Short descriptive world-building passage about space in the story                                                                                                                                                                     \\ \hline
LW & Science Fiction        & Write a new name for a post-modern steampunk dystopian New York City                                                                                                                                                                  \\ \hline
NM & Fantasy & Come up with a fictitious name for a Swiss hotel \\ \hline
GS & Historical Fiction     & \begin{tabular}[c]{@{}l@{}}Write the scene in which Walter Benjamin kills himself with morphine tablets in a spare room at the\\ French-German border in 1940 while escaping from the Nazis. Make unusual observations\end{tabular} \\ \hline
MC & Thriller               & Write a Hollywood action style revenge fantasy against the owner of the knicks                                                                                                                                                        \\ \hline
MG & Horror Mystery         & What are plants that would be in a haunted garden?                                                                                                                                                                                    \\ \hline
MG & Horror Mystery         & \begin{tabular}[c]{@{}l@{}}Write five scariest sentences you can think of related to this short story in the literary horror genre.\end{tabular}                                                                             \\ \hline
MG & Horror Mystery         & Re-write it but make it much more scary. focus on psychological horror aspects.                                                                                                                                                       \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{genre}Instructions pertaining to genre specific writing}
\vspace{-4ex}
\end{table}
Based on our interaction data, we observe that participants who chose to write in a particular genre typically used the LLM to either adhere to the specific style representing that genre or used it for \textit{World Building}. World-building often refers to the creation of a world that is different from our own. We can see this most obviously in genres like fantasy, horror, or science-fiction, where the writer has created something new and exciting for the reader to delve into. Similarly, spy thrillers although usually set in our known world, are also doing a heavy amount of world-building. As can be seen in Table \ref{genre} how KK desired for the model to adapt to the style of \textit{Cormac Mcarthy} who is famously known for his short stories spanning the Western and post-apocalyptic genres. Similarly, MG expected the model to know and adapt to the specifics of the psychological horror genre. Other examples show how participants use the model for world-building either by instructing to draft a genre-specific scene (Table \ref{genre} Row 2,5,6) or simply suggestions of characters/elements that make the world believable at the sensory level (Table \ref{genre} Row 3,4,7)

\subsection{Are writers good prompt engineers?}
Creating effective prompts for Large Language Models (LLMs) might seem simple, but it necessitates understanding the situations where these LLMs make mistakes. To address these errors, one must develop targeted prompting methods and then rigorously evaluate how well those methods work. Recent work \citet{10.1145/3544548.3581388} shows how non-Non-AI experts struggle to design effective prompts to elicit desired behaviors from LLMs. This is an important consideration for the success of our experiment. Based on the interaction data we observed several participants were successfully able to design expressive and high-quality prompts. Some of these prompt designs were inspired by our provided templated prompts as can be seen in Table \ref{promptinsp}. At the same time, we noticed several participants to be very expressive and innovative in coming up with novel prompts to steer the story-writing process. Table \ref{nontemplated} shows some examples of some well-engineered prompts from our participants. 

\begin{table}[!ht]
\def\arraystretch{1.15}
\centering
\small
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{{\color{ao}Rewrite the following text with more rich imagery}: \textit{The rooms were cozy, the food hearty.......}}                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{SH}  & \begin{tabular}[c]{@{}l@{}}Rewrite the following text with more rich and less cliche imagery, taking into account the tone and aesthetics of the piece\\ so far: \textit{People were breathing altogether .....}\end{tabular}                                                                                 \\ \hline
\multicolumn{1}{|l|}{RH}  & \begin{tabular}[c]{@{}l@{}}Rewrite the following text so that it better portrays the characters' emotional turmoil and the gradual deterioration of\\ their judgment
and sanity: \textit{Laura's voice quivered with frustration......}\end{tabular}                                                        \\ \hline
\multicolumn{1}{|l|}{ATF} & Rewrite the following text with more imagery like Mary Shelley's in Frankenstein: ....                                                                                                                                                                                                               \\ \hline\hline
\multicolumn{2}{|l|}{{\color{ao}Elaborate the following text. Add more details}: And he told them that he had once blackmailed a CEO}                                                                                                                                                                                                        \\ \hline
\multicolumn{1}{|l|}{ATF} & \begin{tabular}[c]{@{}l@{}}Elaborate the following text by one sentence. Add a transition to the rest of the story draft: \textit{It may not have been} \\\textit{on a dreary night of November....}\end{tabular}                                                                                                      \\ \hline
\multicolumn{1}{|l|}{RH}  & \begin{tabular}[c]{@{}l@{}}Elaborate the following text. Add more details in which Laura and James take more precautions and thoroughly investigate\\ the Oracle's credibility before trusting them: \textit{In their a quest to end the reign their deep fake avatars, Laura and James....}\end{tabular} \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{promptinsp}Example prompts inspired from our templated propts}
\end{table}

\end{comment}


\begin{table}[!ht]
\def\arraystretch{1.15}
\centering
\small
\begin{tabular}{|l|L{13cm}|}
\hline
\multirow{3}{*}{SH}  & Let's have maggie be the chosen one as this story is ending, how do we get there?                                            \\ \cline{2-2}
& She still dies, but in like a "chosen sacrificial lamb" way, try again               \\ \cline{2-2}
& Her having super powers here is a little too "Carrie", let's have her be a little bit more grounded in reality even if the reckoning isnt, try again                             \\ \hline

\multirow{3}{*}{NM}  & What is the "something extraordinary" the four friends create? Can you be more specific?                                       \\ \cline{2-2}
& Could you suggest a possibility? I want to make it easier for the reader.               \\ \cline{2-2}
& I like that idea. How about one of the friends, Max, is unsatisfied with the project but doesn't know how to tell his friends or back off? Please elaborate                            \\ \cline{2-2}
& Please try again. Max isn't unsure about his own abilities—he doubts whether his friends are in earnest about their artistic intentions. \\ \hline
\end{tabular}
\vspace{2ex}
\caption{ Chaining instructions together for more complex subtasks during writing collective brainstorming}
\label{tab:subtasks}
\vspace{-4ex}
\end{table}

\subsection{Learning to better infer writer intentions can improve suggestion quality}
An advantage of our design choice to maintain the history of interactions (\Cref{sec:draft_chat}) is that it allows the writers to chain instructions in sequence, asking the model to make further edits on the initially generated output. From \Cref{tab:subtasks}, we see that this allows users to use the interaction with the model as a sandbox to brainstorm ideas and execute complex subtasks as part of the writing process. As noted by ES, \emph{``Having a second intelligence in the writing process is a sure way to counter writer's block. If I find myself uncertain with the next step in a story, I can always ask the AI, and even if I don't like the AI's ideas, that kind of dialectic often gets ideas flowing.''} 

However, our writers also highlight that this iterative process becomes frustrating if the LLM fails to understand their intentions. This was noted in the feedback by NM, \emph{``It mostly felt as though I was fighting against the AI to produce what I wanted, instead of the AI helping me"}, and ES, \emph{``The more time spent working with the AI, the interesting its responses get, but this almost defeats its own purpose when it feels more satisfying to the writer to just do what they know they want to do instead of asking the AI to be original."} A future research direction to improve suggestion quality could be to better model a human reader to comprehend the text as noted by MG, 
\emph{``It would be cool if the ChatGPT could act more human and actually understand the writing on the page and then it could be of help but because it doesn't truly understand its help is always going to remain surface-shallow.''} This echoes recent concerns on the inability of current LLMs to reason about the mental states of others when generating text \cite{sap2022neural, sclar-etal-2023-minding,shapira2023clever}. 


\section{Limitations}
\label{sec:limitations}
We highlight several limitations of our study to inform future directions of research. 
We sought feedback from the writers in the initial development of the interface but did not experiment with other forms of writing assistance which conditions our findings to this mode of interaction. It is unclear if more involved assistance in the text editor would lead to a better writing experience. We also provide only a limited set of templates which could bias some participants to using these. Our templates mostly include translation and feedback-based instructions as planning tends to be more specific to each story. 
As discussed in \Cref{sec:model_choice}, we are also limited by the choice of language model. Since GPT-3.5 is a \emph{limited-access} model \citet{liang2022holistic}, we are only able to make inferences connecting our findings to the publicly available training information which does not include any of the data used to train the model. The cost of access also does not allow us to perform interventional experiments to fine-tune the model based on specific user feedback which could result in more helpful suggestions. 

We recruit participants from university mailing lists which results in a pool of candidates who both have formal training in writing as well as an interest to explore the capabilities of generative AI. While we ensure a diverse pool of writers within this pool, further investigation is needed to identify if our findings generalize to a broader pool of writers. Finally, our writers only interact with the model for a limited amount of time (a maximum of three stories) and it is unclear if familiarizing themselves with the capabilities of the model over an extended period could lead to them obtaining more effective assistance through better prompting. 

==> table_with_names.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.35}
\begin{tabular}{|l|c|c|l|}
\hline
Name                   & Abbreviation & Stories Written & Institution                            \\ \hline
Melita Granger         & MG           & 2 &\multirow{8}{*}{School of Arts, Columbia University}   \\ \cline{1-3}
Sam Hennessee          & SH           & 3 &                                       \\ \cline{1-3}
Micah Cash             & MC           & 3 &                                       \\ \cline{1-3}
Ethan Smestad          & ES           &  3 &                                      \\ \cline{1-3}
Allison Theresa Fowler        & ATF           & 3 &                                       \\ \cline{1-3}
Kai-Lilly Karpman      & KK           &  1 &                                      \\ \cline{1-3}
Rhoni Erika Blankenhorn      & REB           & 1 &                                       \\ \cline{1-3}
Caleb Knight           & CK           &   1 &                                     \\ \cline{1-3}
Alexander Thomas Kapsidelis   & ATK           &  1 &                                      \\ \hline\hline%\cline{1-3}
%Anonymous   & Anon          & 3  &      \\ \hline\hline
Nicolas Maurokefalidis & NM           & 2 &\multirow{2}{*}{Iowa Writers Workshop} \\ \cline{1-3}
Logan Hoffman-Smith    & LHS          &   1 & \\ \cline{1-3}
Michael Kaplan    & MK          &   1 & \\ \hline\hline
Falaks Vasa &   FV         & 2 &\multirow{1}{*}{Literary Arts, Brown University} \\ \cline{1-3}\hline\hline
Gabriel Schicchi  &   GS         & 1 &\multirow{1}{*}{The Writing Seminars
, Johns Hopkins University} \\ \cline{1-3} 
\hline\hline
Alex Foster & AF           & 1 &\multirow{2}{*}{NYU, Graduate School of Arts and Science} \\ \cline{1-3}
Ronnie Huett    & RH          &   1 & \\ \cline{1-3}
\hline\hline
Anonymous   & Anon          & 3  &      \\ \hline%\hline
\end{tabular}
\vspace{2ex}
\caption{\label{participants} Participants from 5 MFA Writing programs with the US, recruited for our collaborative story writing experiment}
\end{table*}
